Information Rate-Harvested Power Tradeoff in THz SWIPT Systems Employing Resonant Tunnelling Diode-based EH Circuits

In this paper, we study THz simultaneous wireless information and power transfer (SWIPT) systems. Since coherent information detection is challenging at THz frequencies and Schottky diodes may not be efficient for THz energy harvesting (EH) and information detection, we employ unipolar amplitude shift keying (ASK) modulation at the transmitter (TX) and a resonant tunnelling diode (RTD)-based EH circuit at the receiver (RX) to extract both information and power from the RX signal. We model the dependence of the instantaneous output power at the RX on the instantaneous received power by a non-linear piecewise function, whose parameters are adjusted to fit circuit simulation results. To determine the rate-power tradeoff in THz SWIPT systems, we derive the distribution of the TX signal that maximizes the mutual information between the TX and RX signals subject to constraints on the required average harvested power at the RX and the peak signal amplitude at the TX. Since the computational complexity of maximizing the mutual information may be too high for real-time THz SWIPT systems, for high and low required average harvested powers, we also obtain the suboptimal input signal distribution that maximizes the achievable information rate numerically and in closed form, respectively. Furthermore, based on the obtained results, we propose a suboptimal closed-form TX distribution which also achieves a desired harvested power at the RX. Our simulation results show that a lower reverse current flow and a higher breakdown voltage of the employed RTD are preferable when the input signal power at the RX is low and high, respectively. Finally, we demonstrate that for low and high received signal powers, the rate-power tradeoff of THz SWIPT systems is determined by the peak amplitude of the TX signal and the maximum instantaneous harvested power, respectively.

==> ElectricalCircuit.tex <==






\begin{comment}
	We note that an RTD has multiple quantum barriers, and thus, the I-V characteristic of an RTD includes regions with negative resistance \cite{Villani2021, Clochiatti2020}.
	Specifically, in contrast to Schottky diodes, the current flow $I_\text{d}$ through the diode is not a monotonic increasing function of the applied voltage $U_\text{d}$, but the corresponding I-V curve may have multiple critical points, as, e.g., points\footnotemark\hspace*{0pt} $U^1_\text{d}$ and $U^2_\text{d}$ in Fig.~\ref{Fig:IV_Curve}.
	Furthermore, for high input powers, the reverse-bias applied voltage $U_\text{d}$ may exceed the breakdown voltage $U_\text{d}^\text{br}$ and damage the device \cite{Clochiatti2020}.
	\footnotetext{When the RTD is driven into the region of negative resistance, i.e., when $U_\text{d} \in [U^1_\text{d}, U^2_\text{d}]$, the RTD exhibits an additional RF gain \cite{Clochiatti2020}. The analysis of the impact of this RF gain on the efficiency of EH and information decoding is an interesting direction for further research and is beyond the scope of this paper.}
	Since the current flow of an RTD depends on the signal frequency and is determined by quantum processes, an accurate analytical characterization of the I-V characteristic of an RTD may not be possible \cite{Villani2021, Clochiatti2020}. 
	Therefore, for our numerical results in Section IV, we employ the triple-barrier RTD design that was developed in \cite{Clochiatti2020} and fits the measured\footnotemark\hspace*{0pt} I-V characteristic and S-parameters of the diode designed in \cite{Clochiatti2020}, see Fig.~\ref{Fig:IV_Curve}. 
	\footnotetext{We note that the discrepancy between the RTD I-V characteristic and measurement data for $U_\text{d} \in [U_\text{d}^1, U_\text{d}^2]$ in Fig.~\ref{Fig:IV_Curve} is caused by non-idealities (parasitic oscillations) of the measurement setup adopted in \cite{Clochiatti2020}.}
	
	\begin{figure}[!t]
	\centering
	\includegraphics[draft = false, width=0.7\textwidth]{RtdModel}
	\caption{I-V characteristic of the triple-barrier RTD design in \cite{Clochiatti2020} (blue solid line) matched to the measurement data in \cite{Clochiatti2020} (green dotted line).}
	\label{Fig:IV_Curve}
	\end{figure}
\end{comment}




==> ProofCorollaryOptimal.tex <==
To obtain (\ref{Eqn:OutputPdfAchievable}), we express the output pdf $f_y^\text{ach}(y; f^\text{ach}_x)$ as follows:%\vspace*{-5pt}
\begin{align}
	f_y^\text{ach}(y; f^\text{ach}_x) &= \int_{0}^{\sqrt{\bar{P}_\text{max}}} f^\text{ach}_x(x) f_n(y-x) \text{d}x \nonumber \\	
	& \begin{aligned}
		= \int_{0}^{\sqrt{\bar{P}_\text{max}}} \frac{1}{\sqrt{2 \pi \sigma^2}} &\exp \Big( - \mu_0 \\ &+ \mu^2_1 \frac{x^2}{\bar{P}_\text{\upshape max}}-\frac{ (y-x)^2}{2 \sigma^2} \Big) \text{d}x
	\end{aligned} \nonumber \\
	& \begin{aligned}
		=& \mu_4^{-1} \exp\Big( \frac{y^2}{\bar{P}_\text{\upshape max}} \frac{\mu_1^2}{\mu_4^2} - \mu_0\Big) \\ &\Big[ Q\Big(\frac{y - \mu_4^2 \sqrt{\bar{P}_\text{\upshape max}}}{\mu_4 \sigma}  \Big) - Q\Big(\frac{y}{\mu_4 \sigma}\Big) \Big]%\vspace*{-3pt}
	\end{aligned}
\end{align}
This concludes the proof.

==> ProofCorollaryUniform.tex <==
First, we express the pdf $f_y^\text{ach}$ of the output signal $y = x+n$ in (\ref{Eqn:OutputPdf}) as follows:
\begin{align}
	f_y^\text{ach}(y; f_x^\text{ach}) &=\int_{-\infty}^{\infty} f^\text{ach}_x(x) f_n(y-x) \text{d} x \nonumber \\ &= \int_{0}^{ \sqrt{\bar{P}_\text{\upshape max}} } \frac{1}{\sqrt{\bar{P}_\text{max}}} f_n(y-x) \text{d} x.
	\label{Eqn:Prop5Eqn1}
\end{align}
Since $n$ is a zero-mean Gaussian random variable with variance $\sigma^2$, we have $\int_{0}^{\sqrt{\bar{P}_\text{\upshape max}}} f_n(y-x) \text{d} x = Q\big(\frac{y-\sqrt{\bar{P}_\text{\upshape max}}}{\sigma}\big) - Q\big(\frac{y}{\sigma}\big) $.
This concludes the proof.

==> ProofEquivalentModel.tex <==
Let us consider a distribution with pdf $f_s \in \mathcal{F}_{s}$, which has a mass point at $\tilde{s} \in \mathcal{S}$.
We note that there exists a point $\bar{s} \notin \mathcal{S}$ and $\bar{s} \leq \tilde{s}$, that yields the same information signal $x=\sqrt{\psi( |hs|^2) }$ as $\tilde{s}$, i.e., $\sqrt{\psi( |h\bar{s}|^2) } = \sqrt{\psi( |h\tilde{s}|^2) }$, as shown in Fig.~\ref{Fig:EH_ModelEquiv}.
Thus, for any such distribution $f_s$, an equal or larger value of $\bar{P}_\text{s}(\cdot)$ and $I_s(\cdot)$ can be attained by removing the mass point $\tilde{s}$ and increasing the probability of $\bar{s}$ by $f_s(\tilde{s})$.
Since the new probability is in $\mathcal{F}_{s}$, there exists an optimal input pdf $f_s^\text{opt}$ as solution of (\ref{Eqn:GeneralOptimizationProblem}) that does not have mass points in $\mathcal{S}$. This concludes the proof.

==> ProofFeasibility.tex <==
We note that for a given maximum transmit signal amplitude $\bar{A}$, the instantaneous harvested power can not exceed $\bar{P}_\text{\upshape max}$.
Then, the average power harvested at the RTD-based RX is upper-bounded by $\max_{f_s \in {\mathcal{F}}_{s}} \bar{P}_\text{s}(f_s) = \bar{P}_\text{\upshape max}$.
Thus, for any $\bar{P}_\text{req} > \bar{P}_\text{\upshape max}$, a solution of (\ref{Eqn:GeneralOptimizationProblem}) does not exist.
On the other hand, for any $\bar{P}_\text{req} \in[0,  \bar{P}_\text{\upshape max}]$, there exists at least one pdf $f^1_s = \delta(s-s_0) \in \mathcal{F}_{ s }$ that satisfies constraint (\ref{Eqn:GeneralOptConstr1}) with equality, where $s_0 \leq {\bar{A}}$ is chosen such that $\psi(|hs_0|^2) = \bar{P}_\text{req}$.
This concludes the proof.

==> ProofLemmaEPI.tex <==
The proof follows \cite[Appendix A]{Lapidoth2009}.
Specifically, we express the maximum mutual information in  (\ref{Eqn:RefOutputOptimizationProblem}) as follows:%\vspace*{-3pt}
\begin{align}
	I^*_{\bar{\mathcal{F}}_{x } } &\triangleq \max_{f_x \in \bar{\mathcal{F}}_{ x }} \; I_x(f_x) = \max_{f_x \in \bar{\mathcal{F}}_{ x }} \; h_y(f_x) - h_{n} \\
	&\geq \max_{f_x \in \bar{\mathcal{F}}_{ x }} \; \frac{1}{2} \ln \big( e^{2 h_x(f_x)} + e^{2 h_n} \big) - h_{n} =  J^*_{\bar{\mathcal{F}}_{x} },%\vspace*{-3pt}
\end{align}
\noindent where $h_{y}(f_x)$ and $h_{n} = \frac{1}{2} \ln (2 \pi e \sigma^2)$ are the differential entropies of $y$ for a given pdf $f_x \in \bar{\mathcal{F}}_{ x }$ and AWGN $n$ in (\ref{Eqn:MutualInformation}), respectively.
This concludes the proof.

==> ProofProposedMI.tex <==
First, we express the entropy of random variable $x$, which follows pdf $f_x^\text{cf}(x)$ in (\ref{Eqn:ClosedFormPdfX}), as follows:%\vspace*{-3pt}
\begin{align}
	h_x(f_x^\text{cf}) &%= -\int_0^{\sqrt{\bar{P}_\text{max}}} f_x^\text{cf}(x) \ln f_x^\text{cf}(x) \, \text{d}x 
	= -\int_0^{\sqrt{\bar{P}_\text{max}}} \alpha \bar{P}_\text{max}^{-\frac{\alpha}{2}} x^{\alpha-1} \ln (\alpha \bar{P}_\text{max}^{-\frac{\alpha}{2}} x^{\alpha-1}) \, \text{d}x \nonumber \\
	&%= -\int_0^{1} \alpha y^{\alpha-1} \ln (\alpha \bar{P}_\text{max}^{-\frac{1}{2}} y^{\alpha-1}) \, \text{d}y 
	 =-\int_0^{1} (\alpha-1) \ln y \,\text{d}y^\alpha  -\int_0^{1} \ln (\alpha \bar{P}_\text{max}^{-\frac{1}{2}} ) \, \text{d}y^\alpha \nonumber \\
	 &= \frac{\alpha-1}{\alpha} - \ln\frac{\alpha}{\sqrt{\bar{P}_\text{max}}}.%\vspace*{-3pt}
	\label{Eqn:Col2Eqn1}
\end{align}
Then, to obtain (\ref{Eqn:CF_AchievableRate}), we substitute (\ref{Eqn:Col2Eqn1}) into the definition of achievable rate $J_x(f_x^\text{cf})$ in Lemma~\ref{Lemma:EPI}.
This concludes the proof.


==> ProofUniformDistribution.tex <==
First, we note that if the average power constraint (\ref{Eqn:RefOutputOptConstr1}) in the definition of $\bar{\mathcal{F}}_{x}$ is not present, the differential entropy $h_x(f_x)$, and hence, function $J_x(f_x)$ with $f_x \in \bar{\mathcal{F}}_{x}$ are maximized if the pdf of $x$ is uniform and given by $f_x^\text{ach}$ \cite{Lapidoth2009}.
Furthermore, in this case, the maximum achievable information rate and the average harvested power can be expressed as $J_x(f_x) = J^*_{\bar{\mathcal{F}}_{x}}$ and $\bar{P}_\text{\upshape req} = \mathbb{E}_x\{x^2\} = \frac{1}{3} \bar{P}_\text{\upshape max}$, respectively.
Thus, for $\bar{P}_\text{\upshape req} \in [0, \frac{1}{3} \bar{P}_\text{\upshape max}]$, for the maximization of $J_x(\cdot)$, constraint (\ref{Eqn:RefOutputOptConstr1}) can be relaxed and the optimal distribution of $x$ that yields $J^*_{\bar{\mathcal{F}}_{ x }}$ can always be obtained.
This concludes the proof.

==> SystemSetup.tex <==



In Fig.~\ref{Fig:Results_Tradeoffs}, we plot the mutual information and average harvested power for different values of the maximum amplitude of the transmitted signal ${ \bar{A} }$.
To this end, for different values of required harvested power $\bar{P}_\text{harv}^\text{req} \in [0, \frac{1}{3} \bar{P}_\text{\upshape max}]$ and $\bar{P}_\text{harv}^\text{req} \in [\frac{1}{3} \bar{P}_\text{\upshape max}, \bar{P}_\text{\upshape max}]$, we first obtain the maximum achievable rates $J^*_{\bar{\mathcal{F}}_{ \bar{A} }}$ in Propositions~\ref{Prop:UniformDistribution} and \ref{Prop:OptimalSolution}, respectively.
Next, for the pdfs $f_s^*$ that yield $J^*_{\bar{\mathcal{F}}_{ \bar{A} }}$, we also plot in Fig.~\ref{Fig:Results_Tradeoffs} the mutual information $I(f_s^*)$.
Also, as a baseline scheme, we adopt Gaussian transmit symbols with mean $\frac{{ \bar{A} }}{2}$ truncated to the interval $[0, { \bar{A} }]$.
In particular, for a given value of ${ \bar{A} }$, the corresponding values of mutual information $I(f_s)$ and average harvested power $\bar{P}_\text{harv}(f_s)$ for the baseline scheme in Fig.~\ref{Fig:Results_Tradeoffs} are obtained by adjusting the variance $\sigma_\text{s}$ of the truncated Gaussian~$f_s$.

\begin{figure}[!t]
	\centering
	\includegraphics[draft = false, width=0.7\textwidth]{Results/Tradeoffs/Results_Tradeoff}
	\caption{Achievable rate-power regions for different values of $\bar{A}$.}
	\label{Fig:Results_Tradeoffs}
\end{figure}
We observe in Fig.~\ref{Fig:Results_Tradeoffs} that for any given required average harvested power $\bar{P}_\text{harv}^\text{req}$, the proposed SWIPT system is able to achieve significantly higher information rates than the baseline scheme.
Thus, we conclude that Gaussian signals are highly suboptimal and an optimal design of the transmit symbol waveform is needed for efficient THz SWIPT.
Furthermore, we also observe in Fig.~\ref{Fig:Results_Tradeoffs} that for all ${ \bar{A} }$ and $\bar{P}_\text{harv}^\text{req}$, the gap between the mutual information $I(f_s^*)$ and the achievable rate $J^*_{\bar{\mathcal{F}}_{ \bar{A} }}$ is small.
We note that for all considered values of ${ \bar{A} }$, both the maximum achievable rate $J^*_{\bar{\mathcal{F}}_{ \bar{A} }}$ and the mutual information $I(\cdot)$ decrease as the required average harvested power increases.
Thus, for any peak amplitude ${ \bar{A} }$, there is a tradeoff between the achievable information rate $J^*_{\bar{\mathcal{F}}_{ \bar{A} }}$ and the harvested power $\bar{P}_\text{harv}(\cdot)$ that is characterized by the rate-power region in Fig.~\ref{Fig:Results_Tradeoffs}.
Moreover, we note that for low maximum transmit signal amplitudes, which satisfy ${ \bar{A} } < \frac{\sqrt{\rho_1}}{|h|}$, both the mutual information and the harvested power grow with ${ \bar{A} }$.
However, if the maximum received power at the RX satisfies $ { \bar{A} } \geq \frac{\sqrt{\rho_1}}{|h|}$, i.e., for ${ \bar{A} } \in \{\SI{0.75}{\volt}, \SI{1}{\volt}\}$ in Fig.~\ref{Fig:Results_Tradeoffs}, the boundary of the rate-power regions does not change, and thus, the tradeoff between the mutual information and average harvested power of the THz SWIPT system is determined by the maximum instantaneous harvested power $\psi(\rho_1)$ in Fig.~\ref{Fig:MatchedEhModel} and not by the value of ${ \bar{A} }$.









